CLIP-SLA: Parameter-Efficient CLIP Adaptation for Continuous Sign Language Recognition

Continuous sign language recognition (CSLR) focuses on interpreting and transcribing sequences of sign language gestures in videos. In this work, we propose CLIP sign language adaptation (CLIP-SLA), a novel CSLR framework that leverages the powerful pre-trained visual encoder from the CLIP model to sign language tasks through parameter-efficient fine-tuning (PEFT). We introduce two variants, SLA-Adapter and SLA-LoRA, which integrate PEFT modules into the CLIP visual encoder, enabling fine-tuning with minimal trainable parameters. The effectiveness of the proposed frameworks is validated on four datasets: Phoenix2014, Phoenix2014-T, CSL-Daily, and Isharah-500, where both CLIP-SLA variants outperformed several SOTA models with fewer trainable parameters. Extensive ablation studies emphasize the effectiveness and flexibility of the proposed methods with different vision-language models for CSLR. These findings showcase the potential of adapting large-scale pre-trained models for scalable and efficient CSLR, which pave the way for future advancements in sign language understanding.

==> sec/extra.tex <==
One significant challenge to advancing sign language research is the lack of large-scale annotated datasets. Many of the existing sign language datasets focus on isolated signs \cite{li2020word,Ronchetti2016,Sincan2020,Sidig2021}. While this type of data is useful for specific applications, such as developing dictionaries, real-world applications of SLR require handling full sentences, as in continuous sign language. \textbf{Deep learning methods for SLR and SLT tasks achieve high performance but require extensive data for training.} Recently, the growing interest in gloss-free SLT has led to the development of several datasets, including How2Sign \cite{duarte2021how2sign}, OpenASL \cite{shi2022open}, BOBSL \cite{albanie2021bbc}, SWISSTXT-NEWS \cite{camgoz2021content4all}, and VRT-NEWS \cite{camgoz2021content4all}. While these datasets are more realistic and diverse, compared to existing CSLR datasets, they lack the gloss annotations crucial for CSLR and gloss-based SLT models. 


Table \ref{tab:datasets} provides a comprehensive summary of publicly available CSLR datasets, highlighting key attributes such as sign language, number of signs, number of unique sentences, number of signers, number of samples, domain, video resolution, total duration, and whether the data was captured in the wild (without restricted recording environment). The RWTH-BOSTON-104 dataset ~\cite{Dreuw2009}, is one of the earliest publicly available CSLR datasets, containing relatively few low-resolution samples recorded in a lab by only three signers. subsequently, several German sign language (GSL) datasets were released, including SIGNUM ~\cite{VonAgris2007} and multiple versions of the RWTH-PHOENIX-Weather dataset ~\cite{Forster2012, Koller2015, Camgoz2018}. SIGNUM has a large set of 19,500 video samples recorded by 25 fluent signers. However, the videos were captured under strict conditions, featuring a dark background with all signers wearing long-sleeve black shirts. The RWTH-PHOENIX-Weather ~\cite{Forster2012} dataset portrayed live weather forecasts from TV broadcasts, which was extended in the widely used RWTH-PHOENIX-Weather-2014 (Phoenix2014) dataset \cite{Koller2015}, with 2,048 signs, 6,841 sentences, and 6,841 samples, covering 12.5 hours. The RWTH-PHOENIX-Weather-2014-T \cite{Camgoz2018} version further refines the gloss annotations with 1,066 signs and 8,257 sentences, also providing spoken language annotations suitable for sign language translation tasks. 
Although the RWTH-Phoenix datasets contain real-life recordings they were recorded by only nine signers in a strict environment with the same background, distance from the camera, and camera angle The Continuous CSL dataset ~\cite{Huang2018} is another popular dataset, having a large set of 25K samples featuring Chinese Sign Language (CSL) recorded by 50 signers. The dataset, however, is limited to only 100 unique sentences, which was remedied in the subsequent CSL-Daily dataset  ~\cite{9578398}, featuring 6,598 unique sentences.  The Continuous GrSL dataset ~\cite{Adaloglou2021}, provides Greek Sign Language (GrSL) videos with only 310 signs recorded in a lab with a green background. The domain of the dataset is limited to governmental services. The ArabSign dataset ~\cite{luqman2022arabsign} covers unified Arabic sign language with a limited set of signs and sentences recorded using a Kinect V2 camera. FluentSigners-50 ~\cite{Mukushev2022} presented Kazakh-Russian sign language videos featuring 50 signers recorded in the wild using a variety of devices and backgrounds. However, the dataset is linguistically limited, as it features only 173 sentences covering 278 glosses.  
The FluentSigners-50~\cite{Mukushev2022} includes Kazakh-Russian sign language videos recorded in realistic settings with various devices and backgrounds by 50 different signers. Although the videos were recorded in diverse environments using various devices and backgrounds, the dataset has linguistic limitations, featuring only 173 sentences with 278 glosses. 

%%%%%%%%%%%%%%%%%%%%%%%%% METHODS %%%%%%%%%%%%%%%%%%%%%%%%%%%
 CLIP (Contrastive Language-Image Pre-training) has emerged as a significant model in multimodal learning, combining vision and language understanding in a unified framework \cite{radford2021learning}. CLIP was trained on a vast collection of image-text pairs using contrastive learning, aligning images and corresponding textual descriptions into a shared embedding space. Given its potential, CLIP has been leveraged in various ways for transfer learning and adaptation to new tasks and domains. Prompt tuning adapts CLIP by learning prompts that are appended to the input text before encoding, optimizing the representation for specific downstream tasks \cite{zhou2022learning, khattak2023maple}. Adapter methods have become popular due to their parameter efficiency and flexibility in fine-tuning. These methods add lightweight neural network modules (adapters) to pre-trained models like CLIP and train only these new components while keeping the base model frozen. Several light-weight adapter methods have been proposed for image understanding including CLIP-Adapter \cite{clip-adapter} and Tip-Adapter \cite{zhang2021tip}. ST-Adapter \cite{st-adapter} extends the concept of adapters to dynamic data, allowing CLIP to process video inputs effectively. It introduces modules that incorporate temporal information into the pre-trained CLIP architecture, making it suitable for tasks like action recognition, video classification, and other video understanding challenges.

 
 Inspired by \cite{st-adapter}, we propose CLIP SL Adaptation (CLIP-SLA), which presents a method that leverages the power of pre-trained CLIP weights with a Vision Transformer (ViT-B) backbone to achieve effective representation learning for CSLR. Since CLIP was originally trained on static images, we add adapter modules to adapt the pre-trained image model to video-based CSLR, as shown in \cref{fig:proposed_framework} (b) \textcolor{red}{Hamzah: what about (a)?}. Two adapters are added to each Transformer layer, before the Multi-Head Self-Attention (MHSA) layer and before the Multi-Layer Perceptron (MLP) block. Each adapter consists of a downsampling layer, a 3D convolution (Conv3D) layer, and an upsampling layer, enabling the model to process spatial-temporal features. The Conv3D within the adapter captures temporal dynamics across frames, making the adapted ViT suitable for video input without modifying the CLIP weights directly. Zero-initialization is used in the adapter convolution layers to allow the adapters to begin with minimal influence on the frozen backbone, then gradually adapt to the CSLR-specific features as training progresses. The applied adaptation method helps in learning essential SL features, such as hand shapes and movement trajectories, with minimal alterations to CLIP’s original visual embeddings. The ViT’s output, which now contains temporal information through the adapters, is passed to a sequence learning module to learn long-term temporal dependencies. Following the previous SOTAs \cite{hu2023corrnet,hu2022temporal,hu2023self}, we adopt 1D convolutions (Conv1D) followed by BLSTM for temporal modeling after the visual backbone, as displayed in \cref{fig:proposed_framework} (a).  To further facilitate the training of the framework, we introduce an auxiliary classifier placed immediately after the ViT encoder which is summed with the VAC loss \cite{Min2021}. 

\begin{figure*}%
    \centering  
    \subfloat[]{{\includegraphics[width=.44\linewidth,valign=c]{figures/CLIP_fullframework2.pdf} }}%
    \quad
    \subfloat[]{{\includegraphics[width=.3\linewidth,valign=c]{figures/adapter.pdf} }}%
    \caption{(a) Overview of the proposed CLIP-SLA framework. The frozen CLIP visual encoder is utilized with adapter blocks. An auxiliary classifier is added after the ViT encoder for extra supervision during training. (b) The structure of the adapted Transformer layer, showing the location of the two adapters placed within each block, and a detailed view of the adapter layers.  }
     \label{fig:proposed_framework}%
\end{figure*}%

%%%%%%%%%%%%%%%%%%%%Experiments %%%%%%%%%%%%%%%%%%%%%
\section{Experiments}
\label{sec:experiments}
%In this section we describe the conducted experiments, we begin by outlining the baseline models. The we present the utilized CSLR benchmark datasets, followed by the evaluation metric and training details. Afterwards, we report an discuss the experimental results. Finaly, we dicuss the ablataion studies and the conducted qualitative analysis.  

\subsection{Baseline and Proposed Models}
\vspace{2mm}\noindent\textbf{Baselines.}
In this section, we briefly describe the baseline models used to benchmark the presented Isharah dataset. Five recent SOTA methods were selected: VAC \cite{Min2021}, SMKD  \cite{Hao2021}, SEN \cite{hu2023self}, TLP \cite{hu2022temporal}, and CorrNet \cite{hu2023corrnet}. Visual alignment constraint (VAC) \cite{Min2021} was proposed to enhance the training of the visual backbone by integrating an auxiliary classifier. This model was further refined in \cite{Hao2021} through self-mutual knowledge distillation (SMKD), enabling the main and auxiliary classifiers to share their weights. Temporal Lift Pooling \cite{hu2022temporal} was presented to capture refined downsized feature maps, which resulted in significant performance gains in comparison to the max pooling and average pooling methods. A self-emphasizing network (SEN) \cite{hu2023self} was presented in which allowed better identification of spatial and temporal representations.  CorrNet \cite{hu2023corrnet} proposed identification and correlation modules to capture local temporal movements, providing a detailed understanding of body trajectories to recognize signs effectively. All baselines share the same network structure consisting of ResNet followed by Conv2D layers and BLSTM. 

%As for the sign language translation task, we train the recent GFSLTVLP \cite{zhou2023gloss} model, which leverages contrastive language-image pre-training and masked self-supervised learning to pre-train the visual and language backbones for sign language translation directly without the need for gloss supervision. The method established remarkable results on the Phoenix2014-T and CSL-Daily datasets. 




\subsection{Datasets and Metric}
We 
To confirm the applicability and effectiveness of the proposed approach, we also conducted experiments on three other large-scale, publicly available datasets: Phoenix2014, Phoenix2014-T and CSL-Daily, in addition to the presented Isharah dataset. Details on the three datasets can be found in Section \ref{sec:related_work}. The Word Error Rate (WER) was used to evaluate the CSLR models, which is the standard metric used for CSLR \cite{hu2023corrnet,chen2023twostream}. WER measures the difference between the predicted sequence and the ground truth by calculating the minimum number of edit operations (insertions, deletions, and substitutions) required to transform one sequence into the other, hence, lower WER indicates better performance. 
%As for the SLT task, following all recent SLT methods \cite{zhou2023gloss,chen2023twostream,9578398}, we report the results using BLEU and ROUGE-L. BLEU compares the predicted translation with reference translations by analyzing the overlap of n-grams (continuous sequences of n words). We use BLEU-1 to BLEU-4, which corresponds to evaluating 1-gram, 2-gram, 3-gram, and 4-gram precision, respectively. ROUGE-L which considers the longest common subsequence  between the predicted and reference sentences. Higher BLEU and ROUGE-L means better recognition. 

%\subsection{Training Details}
%Regarding the training settings, we followed the same training settings reported by the studies \cite{Hao2021,hu2023corrnet} for each model. SMKD and CorrNet were trained for 40 epochs with an effective batch-size of 4, except on the Isharah500, as CorrNet required 80 epochs to converge. As for the GFSLTVLP SLT baseline, an effective batch size of 16 was used for both pre-training and fine-tuning for SLT.    
%We adopt ViT-B/16 with CLIP weights as the visual backbone. The framework was developed using PyTorch, with training conducted on one RTX A6000 GPU and a batch size of two. We follow the same training settings in previous CSLR methods The video frames were resized to 256 × 256 pixels, and random cropping to 224 × 224 pixels was used as an augmentation technique. Additionally, random horizontal flipping (50\%) and temporal rescaling (20\%) were applied. For testing, center cropping at a resolution of 224 × 224 pixels was used.  The models were optimized using the Adam optimizer with a weight decay of ${10}^{-4}$, training for 40 epochs. The initial learning rate was set to ${10}^{-4}$ and reduced by a factor of 5 at epochs 20 and 30.

\subsection{Results}
The models were trained using the training standards adopted in \cite{hu2023corrnet,Min2021,Hao2021}, with 40 epochs and a batch size of two. We compare the performance of the proposed CLIP-SLA with previous SOTA in \cref{tab:results_compare}. Our model demonstrates strong performance with the Phoenix2014, Phoenix2014-T, and CSL-Daily datasets, outperforming all RGB based methods. On the Phoenix2014 and Phoenix2014-T test sets, our model achieves test WERs of 18.8\% and 18.9\%, respectively, outperforming prominent baselines such as CorrNet \cite{hu2023corrnet}, SEN \cite{hu2023self}, and the multimodal methods Co-Sign \cite{Jiao_2023_ICCV} and SignBERTplus \cite{hu2023signbert+}. On the large CSL-Daily dataset, our model also excels with a WER of 25.8\% on the test set, with a significant 4.3 WER reduction compared to the best performing RGB based model CorrNet \cite{hu2023corrnet}. These results highlight the effectiveness of our approach in improving recognition accuracy, establishing our model as a new benchmark in CSLR tasks. 


The results of the CSLR baselines on the Isharah sets are presented in \cref{tab:cslr_results}. Our model demonstrates substantial performance over other baselines, across all subsets of the Isharah dataset. On Isharah-500, our model achieves the lowest error rates, with a test WER of 22.4\% in the signer-independent task and 66.3\% for unseen sentences, outperforming the best baseline SMKD by a significant margin (9.1 WER), showcasing its robustness in scenarios with limited data.  Unlike all the baselines which involved fine-tuning ImageNet-pretrained backbones, our adapted CLIP model was able to leverage its inherent flexibility and pre-learned multi-modal representations effectively. For Isharah-1000, CLIP-SLA obtained a test WER of 21.4\% on signer-independent evaluation and 47.3\% on unseen sentences. On the largest subset, Isharah-2000, our model excels with a test WER of 27.1\% in the signer-independent task and 38.4\% for unseen sentences, indicating its adaptability and robustness when handling large-scale, complex data. These results collectively highlight our model's capability to effectively generalize across varying dataset scales, recording environments and linguistic complexities.


In the signer-independent CSLR task, we note a large difference between the results on the dev and test sets, which is because the test set is four times larger than the dev test (\cref{tab:evalaution_mode_stats}). This implies that all the models could benefit from regularization methods such as early stopping to prevent overfitting the dev set. We also observe that CorrNet struggled with the smaller Isharah-500 dataset, although it is a more advanced model compared to the other baselines. However, as the dataset size increased in Isharah-1000 and Isharah-2000, CorrNet's performance improved significantly, obtaining the lowest WER among the other baselines. This suggests that CorrNet may require more extensive data to fully leverage its advanced architecture and generalize effectively across different signers. 


The results also demonstrate the complexity of the unseen sentence evaluation, as the WERs are relativity high compared to the signer-independent evaluation, emphasizing the challenges in this task, where the model is required to generalize and correctly identify new combinations and transitions of signs, compared to the signer-independent task where the test sentences have been encountered by differnt signers.  We also observe a significant reduction in WERs during the unseen-sentence evaluation as the training data increased with the larger Isharah-1000 and Isharah-2000 sets. This trend can be explained by the fact that larger sets provide more diverse sentence structures and linguistic patterns, allowing the model to learn more effectively and generalize better to new unseen sentences. Among the baselines, SMKD showed strong generalization across new unseen gloss sequences with the lowest WER scores (0.3 difference from our model), which implies that simpler models that are less likely to over-fit the gloss sequences are better suited for this task.

\begin{table}[]
\centering
\caption{Comparison of performance in WER (\%) on the Phoenix2014, Phoenix2014-T, and CSL-Daily datasets. Multimodal approaches are marked with ``\dag''. Our method outperforms all RGB based approaches.}
\label{tab:results_compare}
\footnotesize
\resizebox{\columnwidth}{!}{%

\begin{tabular}{@{}lcccccc@{}}
\toprule
                      & \multicolumn{2}{c}{Phoenix2014} & \multicolumn{2}{c}{Phoenix2014-T} & \multicolumn{2}{c}{CSL-Daily} \\ 
                      & Dev            & Test           & Dev             & Test            & Dev           & Test          \\ \midrule
C2SLR\textsuperscript{\dag} \cite{zuo2022c2slr}    & 20.5           & 20.4           & 20.2            & 20.4            & 31.9          & 31.0            \\
CoSign\textsuperscript{\dag} \cite{Jiao_2023_ICCV}    & 19.7           & 20.1           & 19.5            & 20.1            & 28.1          & 27.2          \\
SignBERTplus\textsuperscript{\dag} \cite{hu2023signbert+}       & 19.9           & 20.0             & 18.8            & 19.9            & -            & -            \\
TwoStreamSLR\textsuperscript{\dag} \cite{chen2023twostream}       & 18.4           & 18.8           & 17.7            & 19.3            & 25.4          & 25.3            \\
VAC  \cite{Min2021}  & 21.2           & 22.3           & -            & -            & -          & -            \\
SMKD \cite{Hao2021}                               & 20.8           & 21.0             & 20.8            & 22.4   & - & - \\
TLP  \cite{hu2022temporal} & 19.7           & 20.8           & 19.4            & 21.2            &   -        &  -           \\

SEN  \cite{hu2023self}  & 19.5           & 21.0           & 19.3            & 20.7            &     -      &   -          \\

AdaBrowse   \cite{hu2023adabrowse}                & 19.6           & 20.7           & 19.5            & 20.6   &  31.2 & 30.7  \\
SSSLR \cite{jang2023self}   & 20.9           & 20.7           & 20.5            & 22.3            & -            & -            \\
CTCA   \cite{guo2023distilling}   & 19.5           & 20.3           & 19.3            & 20.3            & 31.3          & 29.4          \\
CVT-SLR \cite{zheng2023cvt}   & 19.8           & 20.1           & 19.4            & 20.3            & -            & -            \\

CorrNet  \cite{hu2023corrnet}    & 18.8           & 19.4           & 18.9            & 20.5            & 30.6          & 30.1          \\ \midrule
CLIP-SLA (ours)              &  \textbf{18.8}	              &   \textbf{18.9}             & \textbf{18.8}          & \textbf{19.5}            & \textbf{26.1}          & \textbf{25.8}            \\ \bottomrule
%\multicolumn{7}{l}{\footnotesize \textsuperscript{*}Multimodal approaches.} \\

\end{tabular}%
}
\end{table}


%The results of the CSLR baselines are displayed in \cref{tab:cslr_results}, while the results of the SLT baseline are presented in \cref{tab:slt_result}. In the signer-independent CSLR task, although CorrNet is a more advanced model than SMKD, it struggled with the smaller Isharah500 dataset, showing higher WER compared to SMKD. However, as the dataset size increased in Isharah1000 and Isharah2000, CorrNet's performance improved significantly, indicating that it benefits from larger training data. This suggests that CorrNet may require more extensive data to fully leverage its advanced architecture and generalize effectively across different signers.  


 

%We also observe in \cref{fig:errors_per_signer} (a), with signer-independent evaluation, that the majority of errors (65.5\%) were deletion errors, indicating that the model mostly omitted unrecognizable signs from the unseen signers due to differences in signing style or speed. Contrary to  unseen sentence evaluation \cref{fig:errors_per_signer} (b), where the model produced near equal rates of substitution and deletion errors (46.2\% and 48.0\% receptively), which implies that the model often replaced the correct signs with incorrect ones, possibly due to insufficient generalization or overfitting to the training data (where it learned specific patterns that do not generalize well to unseen sentences). 

\begin{table*}[]
\centering
\caption{Comparison of performance in WER (\%) on the presented Isharah sets. Our method outperforms all baselines.}
\label{tab:cslr_results}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}l|cc|cc|cc|cc|cc|cc@{}}
\toprule
     & \multicolumn{4}{|c|}{Isharah-500}                                                       & \multicolumn{4}{c|}{Isharah-1000}                                                      & \multicolumn{4}{c}{Isharah-2000}                                                      \\ \cmidrule(l){2-13}
   \multirow{1}{*}{Method}  & \multicolumn{2}{|c}{Signer   independent} & \multicolumn{2}{c|}{Unseen   sentences} & \multicolumn{2}{|c}{Signer   independent} & \multicolumn{2}{c|}{Unseen   sentences} & \multicolumn{2}{|c}{Signer   independent} & \multicolumn{2}{c}{Unseen   sentences} \\ 
        & Dev                  & Test               & Dev                 & Test               & Dev                 & Test                & Dev                 & Test               & Dev                 & Test                & Dev                 & Test               \\ \midrule
VAC \cite{Min2021}    &      17.6            &          34.1      &       72.3          &            66.6      &       running          &        running        &     running            &         running         &          running       &      running            &      running          &     running           \\
SMKD \cite{Hao2021}    & 19.3                 & 31.5               & 72.5                & 68.0                 & 18.5                & 35.1                & 56.6                & 48.0                 & 23.1                & 39                  & 46.8                & 38.8               \\
TLP \cite{hu2022temporal}    &     running             &        running        &       running          &        running          &   running              &         running       &      running          &           running      &      running           &            running       &                 &               \\
SEN \cite{hu2023self}    &      52.3           &    55.2           &               81.9           &    76.2               &             19.1    &          36.4       &       66.2         &      57.3           &      running           &            running       &             running    &     running           \\
CorrNet \cite{hu2023corrnet} & 50.1                 & 54.9               & 82.3                & 77.8               & 18.8                & 31.9                & 63.7                & 55.0                 & 23.3                & 31.2                & 55.2                & 46.5               \\ \midrule
CLIP-SLA (ours) & \textbf{12.2}	& \textbf{22.4}	& \textbf{71.80}	& \textbf{66.3}	& \textbf{14.20}	& \textbf{21.4}	& \textbf{55.4}	& \textbf{47.3}	& \textbf{21.2}	 & \textbf{27.1}	& \textbf{45.3}	& \textbf{38.4} \\

\bottomrule
\end{tabular}%
}
\end{table*}

%\begin{figure*}%
 %   \centering
   
  %  \subfloat[ Signer independent evaluation.]{{\includegraphics[width=5cm,height=5cm]{figures/signerIndp (1).pdf} }}%
   % \qquad
    %\subfloat[Unseen sentence evaluation.]{{\includegraphics[width=5cm,height=5cm]{figures/unseen_sent.pdf} }}%
    %\caption{CSLR performance of each signer in the Isharah2000 test set, showing the percentage of correctly identified sentences, and the percentages of substitution, deletion, and insertion errors. }
 %    \label{fig:errors_per_signer}%
%\end{figure*}%

%\begin{table*}[]
%\centering
%\caption{Results of SLT baseline (Bn: BLEU-n)}.
%\footnotesize
%\label{tab:slt_result}
%\begin{tabular}{@{}c|ccccc|ccccc@{}}
%\toprule
 %           & \multicolumn{5}{c|}{Dev}                 & \multicolumn{5}{c}{Test}                \\ 
  %        Subset  & B1    & B2    & B3    & B4    & ROUGE-L & B1    & B2    & B3    & B4    & ROUGE-L \\ \midrule
%Isharah500  & 68.02 & 66.38 & 65.39 & 64.83 & 69.18   & 47.83 & 45.85 & 44.61 & 43.49 & 49.56   \\
%Isharah1000 & 61.08 & 59.13 & 57.84 & 56.66 & 62.83   & 44.34 & 42.01 & 40.63 & 39.44 & 45.19   \\
%Isharah2000 & 58.73	& 56.65	& 55.22 &	54.00	& 60.71	& 34.59	& 32.41	& 31.09	& 30.20	& 35.86      \\ %\bottomrule
%\end{tabular}%
%\end{table*}

%As for the SLT baseline, we note a decline in BLEU and ROUGE-L score as the dataset size grows. This indicates that the model’s ability to retain sequential coherence is affected by the increased complexity and vocabulary diversity in larger subsets. A BLEU-4 of 30.2\% was obtained on the largest set (Isharah2000). This reflects a solid baseline for gloss-free SLT given the large vocabulary (2690 words) and high number of singletons (1441). High vocabulary diversity (unique words) in a relatively small number of sentences generally increases the difficulty of learning accurate mappings, especially for n-grams. It’s challenging for the model to learn longer, accurate n-gram patterns when there’s high lexical variety and fewer repetitions of word sequences. Augmenting the dataset by generating paraphrased sentences or synthetic data to expose the model to more varied sentence structures would likely improve performance. 

%Finally, in both signer-independent CSLR and SLT tasks, we see a significant drops in performance with the test set compared to the Dev set, especially in larger subsets like Isharah2000. This may indicate a generalization issue where the models struggle to perform as well on unseen data. Hence special attention should be given to improve training such as early-stopping and regularization. 

\subsection{Ablation Studies}
We conduct ablation studies on the Phoenix2014 dataset to validate the effectiveness of the model. 
\par
\vspace{2mm}\noindent\textbf{ Adapter Settings.}
In \cref{tab:adapter_settings}, we investigate several adapter settings to understand the effect of each setting on the overall performance of the CSLR framework. Our initial configuration uses one adapter placed before the MLP block in the Transformer layer, utilizing Conv3D for spatio-temporal modeling. The adapter’s bottleneck width is set to 384, with adapters applied across all 12 layers of the ViT-B/16 backbone. In \cref{tab:adapter_settings} (a), we experimented with two temporal modeling methods: Conv3D with kernel size (3, 1, 1) and Temporal Self-Attention (TSA) with 8 heads. The results show that Conv3D achieves a lower WER compared to Temporal Self-Attention. This indicates that Conv3D is more effective for spatio-temporal feature extraction in this setup, possibly due to better modeling of short-term dependencies, as the TSA layer may have introduced noise from distant frames. Furthermore, Conv3D provides this performance advantage with approximately 6\% fewer parameters, making it both efficient and effective. Therefore, we utilize Conv3D for spatio-temporal modeling throughout the rest of the experiments.  
In \cref{tab:adapter_settings} (b), we investigated different locations of the adapter within the transformer layer, which showed the the adapter positioned before both the MHSA and MLP blocks delivers the best WER performance. This suggests that integrating the adapter at both points allows it to better capture and modulate the information before it flows through the main components of the Transformer block, thus enhancing the temporal and semantic understanding necessary for CSLR. Hence, two adapters are used within each Transformer layer, as illustrated in \cref{fig:proposed_framework}. 


The results with varying adapter widths are presented in \cref{tab:adapter_settings} (c), showing that 256, which reduces the number of channels (768) in the ViT-B by a factor of 3, is the ideal adapter width in our framework. This indicates that this setting provides the right amount of capacity for the model to generalize effectively. To explore the effect of the number of adapter layers and try to find a a balance between performance and efficiency with fewer adapters, we reduced the number of layers in which the adapters were added to the ViT, starting from all 12 layers and removing the adapters at shallower layers.  \cref{tab:adapter_settings} (c) indicates that more adapters across the deeper ViT layers generally boosts performance, due to increased capacity for adaptation to the CSLR task. However, we found that using 11 adapter layers produced the lowest WERs, as reducing the number of adapted layers below this threshold seems to compromise the model's capacity, while adapting more than 11 layers does not yield significant performance improvements.  

\begin{table}[]
\centering
\caption{Comparison of performance in WER (\%) on Phoenix2014 with differnt configuration of the adapter. (a) Type of temporal modeling method implemented in the adapter. (b) Impact of adapter location within the Transformer layer. (c) Effect of different adapter widths. (d) Influence of reducing the number of adapted Transformer layers.}
\label{tab:adapter_settings}
\footnotesize
\begin{tabular}{@{}lll@{}}
\toprule
 Adapter Setting                         & Dev (\%)  & Test (\%)  \\ \midrule
{(a) Temporal Modeling} &      &      \\
\hspace{5mm}Conv3D                    & \textbf{18.9} & \textbf{19.5} \\
\hspace{5mm}TSA & 19.5 & 20.2 \\ \midrule
{(b) Adapter Location}          &      &      \\
\hspace{5mm}Before MHSA                 & 20.5 & 21.2 \\
\hspace{5mm}Before MLP                   & 18.9 & 19.5 \\
\hspace{5mm}Before MHSA and MLP   & \textbf{18.8} & \textbf{19.4} \\ \midrule
{(c) Adapter width}             &      &      \\
\hspace{5mm}192                       & 19.0 & 19.6 \\
\hspace{5mm}256                       & \textbf{18.8} & \textbf{19.1} \\
\hspace{5mm}384                       & 18.8 & 19.4 \\ \midrule
{(d) Adapter Layers}            &      &      \\
\hspace{5mm}12                        & 18.8 & 19.1 \\
\hspace{5mm}11                        & \textbf{18.8} & \textbf{18.9} \\
\hspace{5mm}10                        & 18.9 & 19.1 \\
\hspace{5mm}9                         & 19.0 & 19.4 \\
\hspace{5mm}8                         & 19.2 & 19.5 \\ \bottomrule
\end{tabular}%
\end{table}


\vspace{2mm}\noindent\textbf{Training Strategies.}
\cref{tab:training_methods} provides a comparative analysis of different training methods in terms of parameter efficiency and performance on the Phoenix2014 dataset. The results illustrate the advantages of using our approach over other training methods. Using frozen CLIP weights in our CSLR framework leads to relatively high error rates due to the lack the task-specific adaptability required for effective CSLR. Full fine-tuning resulted in the worst performance likely due overfitting the training data and losing the valuable pre-trained knowledge. On the other hand, fine-tuning only the last layers resulted in better results with significantly fewer parameters compared to the full fine-tuning.  By allowing only the final layers to adapt to the data, the model gains some task-specific learning ability, which reduces the error compared to the frozen setting. However, the inability to update all layers restricts the model’s flexibility. Finally, our approach achieved an optimal balance between performance and efficiency. With only 31 million parameters, our model achieves the best results, demonstrating the effectiveness of the CLIP-SLA method. This setup allows the model to adapt the CLIP weights using spatial and temporal information while maintaining parameter efficiency.

\begin{table}[]
\centering
\caption{Results for using CLIP as the visual encoder in the CSLR framework with different training strategies and the number of trainable parameters in each setting.}
\label{tab:training_methods}
\footnotesize
\begin{tabular}{@{}lllc@{}}
\toprule
Setting                                                  & Dev (\%)   & Test (\%)  & Param (M) \\ \midrule
Frozen                                    & 28.6 & 28.6 & 21.1 \\
Full Fine-tuning                                  & 32.2 & 32.3 & 109.9\\ 
Fine-tuning last layers & 21.0   & 21.6 & 23.2\\ \midrule
% Using CLIP-Adapter \cite{clip-adapter}  &    &  & \\ % investigate it if we have time 
CLIP-SLA (ours)                            & 18.8 & 18.9 & 31.0 \\ \bottomrule
\end{tabular}%
\end{table}

\vspace{2mm}\noindent\textbf{Efficiency Analysis.} \cref{tab:efficiency_analysis} shows an efficiency comparison between our method and the SOTA TwoStreamSLR \cite{chen2023twostream} on the Phoenix2014 dataset. THOP\footnote{https://github.com/ultralytics/thop} was used to compute the GFLOPs using an RTX A6000 GPU with batch size of one. Evidently, our method  achieves a balance between computational efficiency and accuracy, achieving comparable test results to TwoStreamSLR (0.1 WER difference) with 29\% fewer parameters and nearly half the GFLOPs. 

\begin{table}[]
\centering
\caption{Efficiency analysis of our method. }
\footnotesize
\label{tab:efficiency_analysis}
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\toprule
Method          & Dev (\%)   & Test (\%) & Param (M) & GFLOPs \\ \midrule
TwoStreamSLR \cite{chen2023twostream}     & 18.4 & 18.8 & 105.4     & 3,851 \\
CLIP-SLA (ours)             & 18.8 & 18.9 & 31.0      & 1,795 \\ \bottomrule
\end{tabular}%
}
\end{table}

\subsection{Qualitative Results}
To validate the effectiveness of our proposed model and gain deeper insights into the challenges presented in the Isharah-2000 dataset, we compare the gloss predictions with those of the best-performing baselines: the CorrNet baseline for signer-independent evaluation and the SMKD baseline for unseen sentence evaluation. Four representative samples are provided in \cref{tab:qualitative}, with two samples from each evaluation task. In the signer-independent evaluation, the first sample illustrates a deletion error by the CorrNet baseline, which is the most frequent type of error in this task. Specifically, the model failed to recognize and omitted the sign "STRESS". In contrast, our proposed model correctly recognized the sentence. Grad-CAM \cite{selvaraju2017grad} visualizations for both models in \cref{fig:gradcam} reveal that, unlike our method, CorrNet did not focus adequately on the hand movements associated with the sign "STRESS", resulting in the model overlooking the critical features needed to identify the sign. In the second sample, the SMKD baseline confused the sign "ONE" with the sign "PERMISSION". This confusion is likely due to the similarity in hand shapes, as both signs involve an extended index finger with the other fingers retracted. Our model, however, successfully distinguished the subtle differences between the two signs and made the correct prediction. This success can is likely attributed to the pre-trained knowledge and robust representations provided by CLIP. %Additionally, the attention mechanism in CLIP's ViT visual encoder may have allowed our model to focus on critical regions, such as hand and facial movements, more effectively than the CNN-based backbone used in the baselines. This enhanced spatial attention likely contributes to our model’s superior performance in recognizing these challenging signs.


To understand the limitations of our model, we analyzed instances where it  struggled to predict the correct sentence, as displayed in the bottom two samples.  The third sample shows an insertion error, where both models interpreted a motion at the end of the video as an additional sign. This case highlights a common challenge in CSLR, where models must distinguish unintentional gestures from intentional signs. The fourth example illustrates  both models' failure to recognize the sign "MOTORCYCLE", likely due to the sign being partially out of frame. This limitation suggests that the models could benefit from further data augmentation techniques, such as zooming and occlusion, to help them learn to interpret signs even when the full spatial context is unavailable.

\begin{table*}[]
\centering
\caption{Qualitative analysis on Isharah-2000. Deletion, substitution, insertion errors are highlighted in \colorbox{delectblue}{blue}, \colorbox{pink}{pink} and \colorbox{delectgreen}{green}, respectively. }
\label{tab:qualitative}
\resizebox{.8\linewidth}{!}{%
\begin{tabular}{@{}lcc|ccc@{}}
\toprule
Task                        & Signer Independent CSLR                                              & WER (\%)                                   &                                                  & \multicolumn{1}{c}{Unseen Sentence CSLR}                                                    & WER (\%)                        \\ \midrule
\multirow{2}{*}{Sample 1:}       & \textarabic{وجوب خوف توتر ابتعاد}                                     &                  & {\multirow{2}{*}{Sample 2:}}       & {\textarabic{ استئذان غدا عوده}     }                                       &          \\ 
                            & (MUST FEAR STRESS STAY\_AWAY)                                                     &                  &                           &                  (PERMISSION TOMORROW COME\_BACK)                                                                               &        \\ 
\multirow{2}{*}{Pred:}      & \textarabic{وجوب خوف \colorbox{delectblue}{****}  ابتعاد}            & {25.0}              & {\multirow{2}{*}{Pred:}}      & {\textarabic{\colorbox{pink}{واحد} غدا عوده}     }                                           & {33.3}  \\
                            & (MUST FEAR \colorbox{delectblue}{****} STAY\_AWAY )                           &               &                         &           (\colorbox{pink}{ONE} TOMORROW COME\_BACK)                                                                                   &                               \\ 
\multirow{2}{*}{Pred ours:} &        \textarabic{وجوب خوف توتر ابتعاد}                                          &                           \multirow{2}{*}{0.0}             & \multirow{2}{*}{Pred ours:}                      &        {\textarabic{ استئذان غدا عوده}     }                                                                                       &            \multirow{2}{*}{0.0}                \\
                            & \         (MUST FEAR STRESS STAY\_AWAY)                                         &                                        &                                               &      (PERMISSION TOMORROW COME\_BACK)                                                                                          &                                                                                        \\ \midrule
                            
                            
\multirow{2}{*}{Sample 3:}       & \textarabic{ انا سعيد	 سبب زواج صديق ع  ل    ي     }                                       &                  & {\multirow{2}{*}{Sample 4:}}       & \textarabic{دراجه\_ناريه  خطر}                                     &          \\ 
                            & (I HAPPY REASON MARRIAGE FRIEND   A L I)                                                &                  &                           &                  (MOTORCYCLE  DANGEROUS)                                                                               &        \\ 
\multirow{2}{*}{Pred:}      & \textarabic{انا سعيد سبب زواج صديق ع ل ي \colorbox{delectgreen}{يوجد}}           & {12.5}              & {\multirow{2}{*}{Pred:}}      &  \textarabic{ \colorbox{pink}{حقيبه\_يد}  خطر}                                         & {50.0}  \\
                            & (I HAPPY REASON MARRIAGE FRIEND A L I \colorbox{delectgreen}{EXIST})                        &               &                         &           ( \colorbox{pink}{ HAND\_BAG} DANGEROUS)                                                                                  &                               \\ 
\multirow{2}{*}{Pred ours:} &        \textarabic{انا سعيد سبب زواج صديق ع ل ي \colorbox{delectgreen}{لا}}                                            &                           \multirow{2}{*}{12.5}             & \multirow{2}{*}{Pred ours:}                      &        \textarabic{\colorbox{pink}{حذاء} خطر}                                                                                              &            \multirow{2}{*}{50.0}                \\
                            &        (I HAPPY REASON MARRIAGE FRIEND   A L I \colorbox{delectgreen}{NO})                                      &                                        &                                               &      (\colorbox{pink}{SHOE}  DANGEROUS)                                   &    \\ \bottomrule


\end{tabular}%
}
\end{table*}

\begin{figure}[]
\centering
\includegraphics[width=\linewidth]{figures/stress_sign_wo_raw.pdf}
\caption{Grad-CAM visualization for the sign "STRESS" with the baseline model (top) and our model (bottom). The baseline model, which omitted the "STRESS" sign in its prediction, shows limited focus on the hand regions. In contrast, our model, which correctly identified the sign, demonstrates concentrated attention on the hand areas, effectively capturing the key hand movements required for accurate recognition.}
\label{fig:gradcam}
\end{figure}

%\begin{figure}[]
%\centering
%\includegraphics[width=.7\linewidth]{figures/sign_one_vs_sign_permission_new.pdf}
%\caption{Visual similarity between the signs "PERMISSION" (left) and "ONE" (right), highlighting the identical use of an extended index finger with other fingers retracted. This similarity in hand shape and orientation can contribute to baseline model confusion during recognition.}
%\label{fig:sign_one_vs_sign_permission}
%\end{figure}


